A phase field model for mass transport with semi-permeable interfaces

In this paper, a thermal-dynamical consistent model for mass transfer across permeable moving interfaces is proposed by using the energy variation method. We consider a restricted diffusion problem where the flux across the interface depends on its conductance and the difference of the concentration on each side. The diffusive interface phase-field framework used here has several advantages over the sharp interface method. First of all, explicit tracking of the interface is no longer necessary. Secondly, the interfacial condition can be incorporated with a variable diffusion coefficient. A detailed asymptotic analysis confirms the diffusive interface model converges to the existing sharp interface model as the interface thickness goes to zero. A decoupled energy stable numerical scheme is developed to solve this system efficiently. Numerical simulations first illustrate the consistency of theoretical results on the sharp interface limit. Then a convergence study and energy decay test are conducted to ensure the efficiency and stability of the numerical scheme. To illustrate the effectiveness of our phase-field approach, several examples are provided, including a study of a two-phase mass transfer problem where drops with deformable interfaces are suspended in a moving fluid.

==> appendices.tex <==
\appendix
\appendixpage
\addcontentsline{toc}{section}{Appendices}\markboth{APPENDICES}{}
\begin{subappendices}
\subsection{Mathematical notations used in the paper}
Mathematical notations used in this paper are follows. Suppose a 2-rank tensor is denoted as $F$, 
its $l_{2}$ norm is $|F|^{2}=\sum F_{ij}^{2}$. 
If $A$ and $B$ are two 2-rank tensors, 
then $(AB)_{ij}=\sum\limits_{k}A_{ik}B_{kj}$ and the double dot product of these two tensors is $A:B=\sum\limits_{ij}A_{ij}B_{ij}$. 
If $\bm{a}$ and $\bm{b}$ are two vectors, the outer pruduct $\bm{a}\otimes\bm{b}$ means 
$(\bm{a}\otimes\bm{b})_{ij}=\bm{a}_{i}\bm{b}_{j}$. $L^{2}$ norm of the smooth function $f$ in the domain $\Omega$, 
$(\int_{\Omega}|f|^{2}\mathrm{d}\bm{x})^{1/2}$, is denoted by $\|f\|_{\Omega}$. 
%and the $L^{2}$ norm on the boundary $w$, $(\int_{\Gamma}|f|^{2}\mathrm{d}s)^{1/2}$, is denoted by $\|f\|_{\Gamma}$. 
If $f$ and $g$ are two smooth functions in $\Omega$, 
$(f,g)$ stands for the inner product of these two functions and it is defined by $(f,g)=\int_{\Omega}fg\mathrm{d}\bm{x}$. 


\subsection{Detail calculation}\label{detail calculation}
For the entropy, we have 
\begin{align}\label{eqn: entropy dissipation}
\frac{\mathrm{d}}{\mathrm{d}t}E_{ent}
&=\int_{\Omega}\mu_{c}(\frac{\partial c}{\partial t}+\bm{u}\cdot\nabla c)\mathrm{d}\bm{x}
\nonumber\\
&=-\int_{\Omega}\mu_{c}\nabla\cdot\bm{j}_{c}\mathrm{d}\bm{x}
\nonumber\\
&=-\int_{\partial\Omega}\mu_{c}\bm{j}_{c}\cdot\bm{n}\mathrm{d}\bm{x}
+\int_{\Omega}\nabla\mu_{c}\cdot\bm{j}_{c}\mathrm{d}\bm{x}
\nonumber\\
&=\int_{\Omega}\nabla\mu_{c}\cdot\bm{j}_{c}\mathrm{d}\bm{x}.
\end{align}

For the kinetic energy, we have 
\begin{align}\label{eqn: kinetic dissipation}
\frac{\mathrm{d}}{\mathrm{d}t}E_{kin}
=&\frac{\mathrm{d}}{\mathrm{d}t}(\frac{1}{2}\int_{\Omega}\rho|\bm{u}|^{2}\mathrm{d}\bm{x})
\nonumber\\
=&\frac{1}{2}\int_{\Omega}\frac{\partial\rho}{\partial t}|\bm{u}|^{2}\mathrm{d}\bm{x}
+\int_{\Omega}\rho\bm{u}\cdot\frac{\partial \bm{u}}{\partial t}\mathrm{d}\bm{x}
\nonumber\\
=&\frac{1}{2}\int_{\Omega}\frac{\partial\rho}{\partial t}|\bm{u}|^{2}\mathrm{d}\bm{x}
+\int_{\Omega}\rho\bm{u}\cdot\frac{\textbf{D}\bm{u}}{\textbf{D}t}\mathrm{d}\bm{x}
+\int_{\Omega}\nabla\cdot(\rho\bm{u})\frac{|\bm{u}|^{2}}{2}\mathrm{d}\bm{x}
\nonumber\\
=&\int_{\Omega}\bm{u}\cdot(\nabla\cdot\sigma_{\eta}+\nabla\cdot\sigma_{\phi})\mathrm{d}\bm{x}
-\int_{\Omega}p\nabla\cdot\bm{u}\mathrm{d}\bm{x}
\nonumber\\
=&-\int_{\Omega}\nabla\bm{u}:(\sigma_{\eta}+\sigma_{\phi})\mathrm{d}\bm{x}
-\int_{\Omega}p\nabla\cdot\bm{u}\mathrm{d}\bm{x}
\end{align}

For the mix energy, we have 
\begin{align*}
&\frac{\mathrm{d}}{\mathrm{d}t}\int_{\Omega}(G(\phi)+\frac{\gamma^{2}}{2}|\nabla\phi|^{2})\mathrm{d}\bm{x}\\
=&\int_{\Omega}\frac{\partial}{\partial t}(G(\phi)+\frac{\gamma^{2}}{2}|\nabla\phi|^{2})\mathrm{d}\bm{x}\\
=&\int_{\Omega}(G^{\prime}(\phi)\frac{\partial\phi}{\partial t}+\gamma^{2}\nabla\phi\cdot\frac{\partial}{\partial t}\nabla\phi)\mathrm{d}\bm{x}\\
=&\int_{\Omega}(G^{\prime}(\phi)\frac{\partial\phi}{\partial t}+\gamma^{2}\nabla\phi\cdot\nabla\frac{\partial\phi}{\partial t})\mathrm{d}\bm{x}\\
=&\int_{\Omega}G^{\prime}(\phi)\frac{\partial\phi}{\partial t}\mathrm{d}\bm{x}+\int_{\partial\Omega}\gamma^{2}\frac{\partial\phi}{\partial\bm{n}}\frac{\partial\phi}{\partial t}\mathrm{d}s-\int_{\Omega}\nabla\cdot(\gamma^{2}\nabla\phi)\frac{\partial\phi}{\partial t}\mathrm{d}\bm{x}\\
=&\int_{\Omega}(G^{\prime}(\phi)-\nabla\cdot(\gamma^{2}\nabla\phi))\frac{\partial\phi}{\partial t}\mathrm{d}\bm{x}
+\int_{\partial\Omega}\gamma^{2}\frac{\partial\phi}{\partial\bm{n}}\frac{\partial\phi}{\partial t}\mathrm{d}s\\
=&\int_{\Omega}\mu_{\phi}\frac{\partial\phi}{\partial t}\mathrm{d}\bm{x}
+\int_{\partial\Omega}\gamma^{2}\frac{\partial\phi}{\partial\bm{n}}\frac{\partial\phi}{\partial t}\mathrm{d}s\\
=&\int_{\Omega}\mu_{\phi}(\frac{\partial\phi}{\partial t}+\bm{u}\cdot\nabla\phi)\mathrm{d}\bm{x}
-\int_{\Omega}\mu_{\phi}\bm{u}\cdot\nabla\phi\mathrm{d}\bm{x}
+\int_{\partial\Omega}\gamma^{2}\frac{\partial\phi}{\partial\bm{n}}\frac{\partial\phi}{\partial t}\mathrm{d}s\\
=&-\int_{\Omega}\mu_{\phi}\nabla\cdot\bm{j}_{\phi}\mathrm{d}\bm{x}
-\int_{\Omega}\mu_{\phi}\bm{u}\cdot\nabla\phi\mathrm{d}\bm{x}
+\int_{\partial\Omega}\gamma^{2}\frac{\partial\phi}{\partial\bm{n}}\frac{\partial\phi}{\partial t}\mathrm{d}s\\
=&\int_{\Omega}\nabla\mu_{\phi}\cdot\bm{j}_{\phi}\mathrm{d}\bm{x}
-\int_{\partial\Omega}\mu_{\phi}\bm{j}_{\phi}\cdot\bm{n}\mathrm{d}s
-\int_{\Omega}(G(\phi)-\nabla\cdot(\gamma^{2}\nabla\phi))\bm{u}\cdot\nabla\phi\mathrm{d}\bm{x}
+\int_{\partial\Omega}\gamma^{2}\frac{\partial\phi}{\partial\bm{n}}\frac{\partial\phi}{\partial t}\mathrm{d}s\\
=&\int_{\Omega}\nabla\mu_{\phi}\cdot\bm{j}_{\phi}\mathrm{d}\bm{x}
-\int_{\Omega}\bm{u}\cdot \nabla G(\phi)\mathrm{d}\bm{x}
+\int_{\Omega}\gamma^{2}\Delta\phi\nabla\phi\cdot\bm{u}\mathrm{d}\bm{x}
-\int_{\partial\Omega}\mu_{\phi}\bm{j}_{\phi}\cdot\bm{n}\mathrm{d}s
+\int_{\partial\Omega}\gamma^{2}\frac{\partial\phi}{\partial\bm{n}}\frac{\partial\phi}{\partial t}\mathrm{d}s\\
=&\int_{\Omega}\nabla\mu_{\phi}\cdot\bm{j}_{\phi}\mathrm{d}\bm{x}
-\int_{\Omega}\bm{u}\cdot \nabla G(\phi)\mathrm{d}\bm{x}
+\int_{\Omega}\gamma^{2}(\nabla\cdot(\nabla\phi\otimes\nabla\phi)
-\frac{1}{2}\nabla|\nabla\phi|^{2})\cdot\bm{u}\mathrm{d}\bm{x}\\
&-\int_{\partial\Omega}\mu_{\phi}\bm{j}_{\phi}\cdot\bm{n}\mathrm{d}s
+\int_{\partial\Omega}\gamma^{2}\frac{\partial\phi}{\partial\bm{n}}\frac{\partial\phi}{\partial t}\mathrm{d}s\\
=&\int_{\Omega}\nabla\mu_{\phi}\cdot\bm{j}_{\phi}\mathrm{d}\bm{x}
-\int_{\Omega}\bm{u}\cdot \nabla (G(\phi)+\frac{\gamma^{2}}{2}|\nabla\phi|^{2})\mathrm{d}\bm{x}
+\int_{\Omega}\gamma^{2}\nabla\cdot(\nabla\phi\otimes\nabla\phi)\cdot\bm{u}\mathrm{d}\bm{x}\\
&-\int_{\partial\Omega}\mu_{\phi}\bm{j}_{\phi}\cdot\bm{n}\mathrm{d}s
+\int_{\partial\Omega}\gamma^{2}\frac{\partial\phi}{\partial\bm{n}}\frac{\partial\phi}{\partial t}\mathrm{d}s\\
=&\int_{\Omega}\nabla\mu_{\phi}\cdot\bm{j}_{\phi}\mathrm{d}\bm{x}
-\int_{\Omega}\nabla\cdot(\bm{u}(G(\phi)+\frac{\gamma^{2}}{2}|\nabla\phi|^{2}))\mathrm{d}\bm{x}
+\int_{\Omega}(G(\phi)+\frac{\gamma^{2}}{2}|\nabla\phi|^{2})\nabla\cdot\bm{u}\mathrm{d}\bm{x}\\
&+\int_{\Omega}\gamma^{2}\nabla\cdot(\nabla\phi\otimes\nabla\phi)\cdot\bm{u}\mathrm{d}\bm{x}
-\int_{\partial\Omega}\mu_{\phi}\bm{j}_{\phi}\cdot\bm{n}\mathrm{d}s
+\int_{\partial\Omega}\gamma^{2}\frac{\partial\phi}{\partial\bm{n}}\frac{\partial\phi}{\partial t}\mathrm{d}s\\
=&\int_{\Omega}\nabla\mu_{\phi}\cdot\bm{j}_{\phi}\mathrm{d}\bm{x}
-\int_{\partial\Omega}(G(\phi)+\frac{\gamma^{2}}{2}|\nabla\phi|^{2}))\bm{u}\cdot\bm{n}\mathrm{d}s
+\int_{\Omega}\gamma^{2}\nabla\cdot(\nabla\phi\otimes\nabla\phi)\cdot\bm{u}\mathrm{d}\bm{x}\\
&-\int_{\partial\Omega}\mu_{\phi}\bm{j}_{\phi}\cdot\bm{n}\mathrm{d}s
+\int_{\partial\Omega}\gamma^{2}\frac{\partial\phi}{\partial\bm{n}}\frac{\partial\phi}{\partial t}\mathrm{d}s\\
=&\int_{\Omega}\nabla\mu_{\phi}\cdot\bm{j}_{\phi}\mathrm{d}\bm{x}
-\int_{\Omega}\gamma^{2}(\nabla\phi\otimes\nabla\phi):\nabla\bm{u}\mathrm{d}\bm{x}, 
\end{align*}
where we use the incompressible condition and boundary condition 
$\bm{u}\cdot\bm{n}|_{\partial\Omega}=0,\bm{j}_{\phi}\cdot{\bm{n}}|_{\partial\Omega}=0,\frac{\partial\phi}{\partial\bm{n}}|_{\partial\Omega}=0.$

Note that
\begin{align*}
|D_{\eta}|^{2}=&\big|\frac{\nabla\bm{u}+(\nabla\bm{u})^{T}}{2}\big|^{2}\\
=&\frac{1}{4}\sum_{i,j}(\partial_{i}u_{j}+\partial_{j}u_{i})^{2}\\
=&\frac{1}{4}\sum_{i,j}\big((\partial_{i}u_{j})^{2}+(\partial_{j}u_{i})^{2}+2\partial_{i}u_{j}\partial_{j}u_{i}\big)\\
=&\frac{1}{4}\sum_{i,j}\big((\partial_{i}u_{j})^{2}+\partial_{i}u_{j}\partial_{j}u_{i}\big)
+\sum_{i,j}\big(\partial_{j}u_{i})^{2}+\partial_{i}u_{j}\partial_{j}u_{i}\big)\\
=&\frac{1}{2}\sum_{i,j}\big((\partial_{i}u_{j})^{2}+\partial_{i}u_{j}\partial_{j}u_{i}\big)\\
=&\frac{1}{2}\sum_{i,j}(\partial_{i}u_{j}+\partial_{i}u_{j}\partial_{j}u_{i})(\partial_{i}u_{j})\\
=&D_{\eta}:\nabla\bm{u}.
\end{align*}

\subsection{}
The following equation is important in derivation of this system. 
\begin{equation}\label{eqn: cross multiply}
\nabla\cdot(\nabla\phi\otimes\nabla\phi)=\Delta\phi\nabla\phi+\frac{1}{2}\nabla|\nabla\phi|^{2}. 
\end{equation}
\begin{proof}
Note that each element of $\nabla\cdot(\nabla\phi\otimes\nabla\phi)$ is 
\begin{equation*}
\partial_{j}(\partial_{i}\phi\partial_{j}\phi)
=\partial_{i}\phi\partial_{jj}^{2}\phi+\partial_{j}(\partial_{i}\phi)\partial_{j}\phi
=\partial_{i}\phi\partial_{jj}^{2}\phi+\partial_{i}(\partial_{j}\phi)\partial_{j}\phi.
\end{equation*}
\end{proof}
\end{subappendices}

%\begin{subappendices}
%%{\color{red}
%\begin{remark}\label{rmk: equivalent of heat equation}
%The following two equations are equivalent.
%\begin{subequations}
%\begin{align}
%&\frac{\partial f}{\partial t}-\nabla\cdot(\frac{Df}{k_{B}T}\nabla\mu_{f})=0,\label{eqn: heat equation}\\
%&\frac{\partial f}{\partial t}-\nabla\cdot(D\nabla f)=0,\label{eqn: reaction-diffuse equation}
%\end{align}
%\end{subequations}
%with the energy(entropy) 
%\begin{equation}\label{eqn: heat equation energy}
%E_{ent}=\int_{\Omega}k_{B}Tf\ln f\mathrm{d}\bm{x}.
%\end{equation}
%\begin{proof}
%The chemical potential is 
%\begin{equation}\label{eqn:heat equation chemical potential}
%\mu_{f}=\frac{\delta E_{ent}}{\delta f}=k_{B}T(\ln f + 1), 
%\end{equation}
%hence we have 
%\begin{equation}\label{eqn: gradient of heat equation chemical potential}
%\nabla\mu_{f}=k_{B}T\frac{\nabla f}{f}, 
%\end{equation}
%and 
%\begin{align*}\label{eqn: energy dissipation}
%\frac{\mathrm{d}}{\mathrm{d}t}E_{ent}
%&=\int_{\Omega}\mu_{f}\frac{\partial f}{\partial t}\mathrm{d}\bm{x}\\
%&=\int_{\Omega}\mu_{f}\nabla\cdot(\frac{Df}{k_{B}T}\nabla\mu_{f})\mathrm{d}\bm{x}\\
%&=\int_{\partial\Omega}\mu_{f}\frac{Df}{k_{B}T}\nabla\mu_{f}\cdot\bm{n}\mathrm{d}\bm{s}
%-\int_{\Omega}\frac{Df}{k_{B}T}|\nabla\mu_{f}|^{2}\mathrm{d}\bm{x}\\
%&=-\int_{\Omega}\frac{Df}{k_{B}T}|\nabla\mu_{f}|^{2}\mathrm{d}\bm{x}.
%\end{align*}
%Here we take the boundary condtion $\nabla\mu_{f}\cdot\bm{n}|_{\partial\Omega}=0$. 
%Combining the conservation law 
%\begin{equation}\label{eqn: conversation law for heat equation}
%\frac{\partial f}{\partial t}+\nabla\cdot(\bm{u}f)=0, 
%\end{equation}
%we have 
%\begin{equation}
%-\frac{Df}{k_{B}T}\nabla\mu_{f}=f\bm{u}, 
%\end{equation}
%i.e. 
%\begin{equation}\label{eqn: relation of mu and u}
%\nabla\mu_{f}=-\frac{k_{B}T}{D}\bm{u}. 
%\end{equation}
%Therefore the energy dissipative law could be expressed as 
%\begin{equation*}
%\frac{\mathrm{d}}{\mathrm{d}t}E_{ent}
%=-\int_{\Omega}\frac{k_{B}Tf}{D}|\bm{u}|^{2}\mathrm{d}\bm{x}.
%\end{equation*}
%This completes the proof.
%\end{proof}
%\end{remark}%}
%
%%{\color{blue}
%\begin{remark}
%A new proof version of Remark \ref{rmk: equivalent of heat equation}. 
%\begin{proof}
%We have the following equation 
%\begin{equation*}
%\frac{\partial f}{\partial t}=-\nabla\cdot\bm{j}_{f}, 
%\end{equation*}
%with the following dissipative law 
%\begin{equation*}
%\frac{\mathrm{d}}{\mathrm{d}t}E_{ent}
%=\frac{\mathrm{d}}{\mathrm{d}t}\int_{\Omega}k_{B}Tf\ln f\mathrm{d}\bm{x}
%=-\int_{\Omega}\eta|\bm{j_{f}}|^{2}\mathrm{d}\bm{x}.
%\end{equation*}
%By carefully calculation, we obtain 
%\begin{align*}
%\frac{\mathrm{d}}{\mathrm{d}t}\int_{\Omega}k_{B}Tf\ln f\mathrm{d}\bm{x}
%&=\int_{\Omega}\mu_{f}\frac{\partial f}{\partial t}\mathrm{d}\bm{x}\\
%&=-\int_{\Omega}\mu_{f}\nabla\cdot\bm{j}\mathrm{d}\bm{x}\\
%&=\int_{\Omega}\nabla\mu_{f}\cdot\bm{j}\mathrm{d}\bm{x}
%-\int_{\partial\Omega}\mu_{f}\bm{j}\cdot\bm{n}\mathrm{d}\bm{s}\\
%&=-\int_{\Omega}\eta|\bm{j}_{f}|^{2}\mathrm{d}\bm{x}.
%\end{align*}
%If we let $\bm{j}=-\frac{1}{\eta}\nabla\mu_{f}$ and $\eta=\frac{1}{Df}$, 
%the following result is observed 
%\begin{equation*}
%\frac{\partial f}{\partial t}-\nabla\cdot(D\nabla f)=0. 
%\end{equation*}
%Here we take the boundary condition $\bm{j}\cdot\bm{n}|_{\partial\Omega}=0$.
%\end{proof}
%\end{remark}%}
%\end{subappendics}
